Binary Morphological Neural Network

In the last ten years, Convolutional Neural Networks (CNNs) have formed the basis of deep-learning architectures for most computer vision tasks. However, they are not necessarily optimal. For example, mathematical morphology is known to be better suited to deal with binary images. In this work, we create a morphological neural network that handles binary inputs and outputs. We propose their construction inspired by CNNs to formulate layers adapted to such images by replacing convolutions with erosions and dilations. We give explainable theoretical results on whether or not the resulting learned networks are indeed morphological operators. We present promising experimental results designed to learn basic binary operators, and we have made our code publicly available online.

==> results_table_dilero.tex <==
     \begin{tabular}{ | c | c | c | c | c | c | c |}
        \hline
        Operation & Disk & Hstick & Vstick & Scross & Dcross & Square \\
        \hline
        Target
        & \begin{minipage}{.12\linewidth}
          \includegraphics[width=\textwidth]{selem_results/true_disk7.png}
        \end{minipage}
        & \begin{minipage}{.12\linewidth}
          \includegraphics[width=\textwidth]{selem_results/true_hstick7.png}
        \end{minipage}
        & \begin{minipage}{.12\linewidth}
          \includegraphics[width=\textwidth]{selem_results/true_vstick7.png}
  
        \end{minipage}
        & \begin{minipage}{.12\linewidth}
          \includegraphics[width=\textwidth]{selem_results/true_scross7.png}
        \end{minipage}
        & \begin{minipage}{.12\linewidth}
          \includegraphics[width=\textwidth]{selem_results/true_dcross7.png}
        \end{minipage}
        & \begin{minipage}{.12\linewidth}
          \includegraphics[width=\textwidth]{selem_results/true_square7.png}
        \end{minipage}
        \\        
        \hline
        Dilation $\dil{}{}$
        & \begin{minipage}{.12\linewidth}
          \includegraphics[width=\textwidth]{selem_results/dilation/dilation_disk7.png}
          \vspace{-1cm}
          \center{{\tiny $1$}}
        \end{minipage}
        & \begin{minipage}{.12\linewidth}
          \includegraphics[width=\textwidth]{selem_results/dilation/dilation_hstick7.png}
          \vspace{-1cm}
          \center{{\tiny $1$}}
        \end{minipage}
        & \begin{minipage}{.12\linewidth}
          \includegraphics[width=\textwidth]{selem_results/dilation/dilation_vstick7.png}
          \vspace{-1cm}
          \center{{\tiny $1$}}
        \end{minipage}
        & \begin{minipage}{.12\linewidth}
          \includegraphics[width=\textwidth]{selem_results/dilation/dilation_scross7.png}
          \vspace{-1cm}
          \center{{\tiny $1$}}
        \end{minipage}
        & \begin{minipage}{.12\linewidth}
          \includegraphics[width=\textwidth]{selem_results/dilation/dilation_dcross7.png}
          \vspace{-1cm}
          \center{{\tiny $1$}}
        \end{minipage}
        & \begin{minipage}{.12\linewidth}
          \includegraphics[width=\textwidth]{selem_results/dilation/dilation_square7.png}
          \vspace{-1cm}
          \center{{\tiny $1$}}
        \end{minipage}
        \\       
        \hline
        Erosion $\ero{}{}$
        & \begin{minipage}{.12\linewidth}
          \includegraphics[width=\textwidth]{selem_results/erosion/erosion_disk7.png}
          \vspace{-1cm}
          \center{{\tiny $1$}}
        \end{minipage}
        & \begin{minipage}{.12\linewidth}
          \includegraphics[width=\textwidth]{selem_results/erosion/erosion_hstick7.png}
          \vspace{-1cm}
          \center{{\tiny $1$}}
        \end{minipage}
        & \begin{minipage}{.12\linewidth}
          \includegraphics[width=\textwidth]{selem_results/erosion/erosion_vstick7.png}
          \vspace{-1cm}
          \center{{\tiny $1$}}
        \end{minipage}
        & \begin{minipage}{.12\linewidth}
          \includegraphics[width=\textwidth]{selem_results/erosion/erosion_scross7.png}
          \vspace{-1cm}
          \center{{\tiny $1$}}
        \end{minipage}
        & \begin{minipage}{.12\linewidth}
          \includegraphics[width=\textwidth]{selem_results/erosion/erosion_dcross7.png}
          \vspace{-1cm}
          \center{{\tiny $1$}}
        \end{minipage}
        & \begin{minipage}{.12\linewidth}
          \includegraphics[width=\textwidth]{selem_results/erosion/erosion_square7.png}
          \vspace{-1cm}
          \center{{\tiny $1$}}
        \end{minipage}
        \\
        \hline
      \end{tabular}


==> results_table_dilero2.tex <==
     \begin{tabular}{ | c | c | c | c | c | c | c | c | c | c |}
        \hline
        Dataset & \multicolumn{3}{c|}{Diskorect}  & \multicolumn{3}{c|}{Mnist} & \multicolumn{3}{c|}{Inverted Mnist} \\
        \hline
        Operation & Disk & Hstick & Dcross & Disk & Hstick & Dcross  & Disk & Hstick & Dcross \\
        \hline
        Target
        & \begin{minipage}{.12\linewidth}
          \includegraphics[width=\textwidth]{selem_results/true_disk7.png}
        \end{minipage}
        & \begin{minipage}{.12\linewidth}
          \includegraphics[width=\textwidth]{selem_results/true_hstick7.png}
        \end{minipage}
        & \begin{minipage}{.12\linewidth}
          \includegraphics[width=\textwidth]{selem_results/true_dcross7.png}
        \end{minipage}
        & \begin{minipage}{.12\linewidth}
          \includegraphics[width=\textwidth]{selem_results2/true_disk5.png}
        \end{minipage}
        & \begin{minipage}{.12\linewidth}
          \includegraphics[width=\textwidth]{selem_results2/true_hstick5.png}
        \end{minipage}
        & \begin{minipage}{.12\linewidth}
          \includegraphics[width=\textwidth]{selem_results2/true_dcross5.png}
        \end{minipage}
        & \begin{minipage}{.12\linewidth}
          \includegraphics[width=\textwidth]{selem_results2/true_disk5.png}
        \end{minipage}
        & \begin{minipage}{.12\linewidth}
          \includegraphics[width=\textwidth]{selem_results2/true_hstick5.png}
        \end{minipage}
        & \begin{minipage}{.12\linewidth}
          \includegraphics[width=\textwidth]{selem_results2/true_dcross5.png}
        \end{minipage}
        \\        
        \hline
        Dilation $\dil{}{}$
        & \begin{minipage}{.12\linewidth}
          \includegraphics[width=\textwidth]{selem_results2/diskorect/dilation/disk.png}
          \vspace{-1cm}
          \center{{\tiny $0$}}
        \end{minipage}
        & \begin{minipage}{.12\linewidth}
          \includegraphics[width=\textwidth]{selem_results2/diskorect/dilation/hstick.png}
          \vspace{-1cm}
          \center{{\tiny $0$}}
        \end{minipage}
        & \begin{minipage}{.12\linewidth}
          \includegraphics[width=\textwidth]{selem_results2/diskorect/dilation/dcross.png}
          \vspace{-1cm}
          \center{{\tiny $0$}}
        \end{minipage}
        & \begin{minipage}{.12\linewidth}
          \includegraphics[width=\textwidth]{selem_results2/mnist/dilation/disk.png}
          \vspace{-1cm}
          \center{{\tiny $0$}}
        \end{minipage}
        & \begin{minipage}{.12\linewidth}
          \includegraphics[width=\textwidth]{selem_results2/mnist/dilation/hstick.png}
          \vspace{-1cm}
          \center{{\tiny $0$}}
        \end{minipage}
        & \begin{minipage}{.12\linewidth}
          \includegraphics[width=\textwidth]{selem_results2/mnist/dilation/dcross.png}
          \vspace{-1cm}
          \center{{\tiny $0$}}
        \end{minipage}
                & \begin{minipage}{.12\linewidth}
          \includegraphics[width=\textwidth]{selem_results2/inverted_mnist/dilation/disk.png}
          \vspace{-1cm}
          \center{{\tiny $0$}}
        \end{minipage}
        & \begin{minipage}{.12\linewidth}
          \includegraphics[width=\textwidth]{selem_results2/inverted_mnist/dilation/hstick.png}
          \vspace{-1cm}
          \center{{\tiny $0$}}
        \end{minipage}
        & \begin{minipage}{.12\linewidth}
          \includegraphics[width=\textwidth]{selem_results2/inverted_mnist/dilation/dcross.png}
          \vspace{-1cm}
          \center{{\tiny $0$}}
        \end{minipage}
        
        \\       
        \hline
        Erosion $\ero{}{}$
        & \begin{minipage}{.12\linewidth}
          \includegraphics[width=\textwidth]{selem_results2/diskorect/erosion/disk.png}
          \vspace{-1cm}
          \center{{\tiny $0$}}
        \end{minipage}
        & \begin{minipage}{.12\linewidth}
          \includegraphics[width=\textwidth]{selem_results2/diskorect/erosion/hstick.png}
          \vspace{-1cm}
          \center{{\tiny $0$}}
        \end{minipage}
        & \begin{minipage}{.12\linewidth}
          \includegraphics[width=\textwidth]{selem_results2/diskorect/erosion/dcross.png}
          \vspace{-1cm}
          \center{{\tiny $0$}}
        \end{minipage}
        & \begin{minipage}{.12\linewidth}
          \includegraphics[width=\textwidth]{selem_results2/mnist/erosion/disk.png}
          \vspace{-1cm}
          \center{{\tiny $0.001$}}
        \end{minipage}
        & \begin{minipage}{.12\linewidth}
          \includegraphics[width=\textwidth]{selem_results2/mnist/erosion/hstick.png}
          \vspace{-1cm}
          \center{{\tiny $0$}}
        \end{minipage}
        & \begin{minipage}{.12\linewidth}
          \includegraphics[width=\textwidth]{selem_results2/mnist/erosion/dcross.png}
          \vspace{-1cm}
          \center{{\tiny $0$}}
        \end{minipage}
        & \begin{minipage}{.12\linewidth}
          \includegraphics[width=\textwidth]{selem_results2/inverted_mnist/erosion/disk.png}
          \vspace{-1cm}
          \center{{\tiny $0$}}
        \end{minipage}
        & \begin{minipage}{.12\linewidth}
          \includegraphics[width=\textwidth]{selem_results2/inverted_mnist/erosion/hstick.png}
          \vspace{-1cm}
          \center{{\tiny $0$}}
        \end{minipage}
        & \begin{minipage}{.12\linewidth}
          \includegraphics[width=\textwidth]{selem_results2/inverted_mnist/erosion/dcross.png}
          \vspace{-1cm}
          \center{{\tiny $0.0001$}}
        \end{minipage}
        \\
        \hline
      \end{tabular}


==> results_table_dilero4.tex <==
     \begin{tabular}{ | c | c | c | c | c | c | c | c | c | c |}
        \hline
        Dataset & \multicolumn{3}{c|}{Diskorect}  & \multicolumn{3}{c|}{MNIST} & \multicolumn{3}{c|}{Inverted MNIST} \\
        \hline
        Operation & Disk & Stick & Cross & Disk & Stick & Cross  & Disk & Stick & Cross \\
        \hline
        Target
        & \begin{minipage}{.12\linewidth}
          \includegraphics[width=\textwidth,left]{selem_results/true_disk7.png}
        \end{minipage}
        & \begin{minipage}{.12\linewidth}
          \includegraphics[width=\textwidth]{selem_results/true_hstick7.png}
        \end{minipage}
        & \begin{minipage}{.12\linewidth}
          \includegraphics[width=\textwidth]{selem_results/true_dcross7.png}
        \end{minipage}
        & \begin{minipage}{.12\linewidth}
          \includegraphics[width=\textwidth]{selem_results2/true_disk5.png}
        \end{minipage}
        & \begin{minipage}{.12\linewidth}
          \includegraphics[width=\textwidth]{selem_results2/true_hstick5.png}
        \end{minipage}
        & \begin{minipage}{.12\linewidth}
          \includegraphics[width=\textwidth]{selem_results2/true_dcross5.png}
        \end{minipage}
        & \begin{minipage}{.12\linewidth}
          \includegraphics[width=\textwidth]{selem_results2/true_disk5.png}
        \end{minipage}
        & \begin{minipage}{.12\linewidth}
          \includegraphics[width=\textwidth]{selem_results2/true_hstick5.png}
        \end{minipage}
        & \begin{minipage}{.12\linewidth}
          \includegraphics[width=\textwidth]{selem_results2/true_dcross5.png}
        \end{minipage}
        \\        
        \hline
        Dilation $\dil{}{}$
        & \begin{minipage}{.12\linewidth}
          \includegraphics[width=\textwidth]{selem_results3/diskorect_dilation_disk.png}
          \vspace{-1cm}
          \center{{\tiny ${0.000}$}}
        \end{minipage}
        & \begin{minipage}{.12\linewidth}
          \includegraphics[width=\textwidth]{selem_results3/diskorect_dilation_stick.png}
          \vspace{-1cm}
          \center{{\tiny ${0.000}$}}
        \end{minipage}
        & \begin{minipage}{.12\linewidth}
          \includegraphics[width=\textwidth]{selem_results3/diskorect_dilation_cross.png}
          \vspace{-1cm}
          \center{{\tiny ${0.000}$}}
        \end{minipage}
        & \begin{minipage}{.12\linewidth}
          \includegraphics[width=\textwidth]{selem_results3/mnist_dilation_disk.png}
          \vspace{-1cm}
          \center{{\tiny ${0.000}$}}
        \end{minipage}
        & \begin{minipage}{.12\linewidth}
          \includegraphics[width=\textwidth]{selem_results3/mnist_dilation_stick.png}
          \vspace{-1cm}
          \center{{\tiny ${0.000}$}}
        \end{minipage}
        & \begin{minipage}{.12\linewidth}
          \includegraphics[width=\textwidth]{selem_results3/mnist_dilation_cross.png}
          \vspace{-1cm}
          \center{{\tiny ${0.000}$}}
        \end{minipage}
                & \begin{minipage}{.12\linewidth}
          \includegraphics[width=\textwidth]{selem_results3/inverted_mnist_dilation_disk.png}
          \vspace{-1cm}
          \center{{\tiny ${0.000}$}}
        \end{minipage}
        & \begin{minipage}{.12\linewidth}
          \includegraphics[width=\textwidth]{selem_results3/inverted_mnist_dilation_stick.png}
          \vspace{-1cm}
          \center{{\tiny ${0.000}$}}
        \end{minipage}
        & \begin{minipage}{.12\linewidth}
          \includegraphics[width=\textwidth]{selem_results3/inverted_mnist_dilation_cross.png}
          \vspace{-1cm}
          \center{{\tiny ${0.000}$}}
        \end{minipage}
        
        \\       
        \hline
        Erosion $\ero{}{}$
        & \begin{minipage}{.12\linewidth}
          \includegraphics[width=\textwidth]{selem_results3/diskorect_erosion_disk.png}
          \vspace{-1cm}
          \center{{\tiny ${0.003}$}}X
        \end{minipage}
        & \begin{minipage}{.12\linewidth}
          \includegraphics[width=\textwidth]{selem_results3/diskorect_erosion_stick.png}
          \vspace{-1cm}
          \center{{\tiny ${0.000}$}}X
        \end{minipage}
        & \begin{minipage}{.12\linewidth}
          \includegraphics[width=\textwidth]{selem_results3/diskorect_erosion_cross.png}
          \vspace{-1cm}
          \center{{\tiny ${0.000}$}}X
        \end{minipage}
        & \begin{minipage}{.12\linewidth}
          \includegraphics[width=\textwidth]{selem_results3/mnist_erosion_disk.png}
          \vspace{-1cm}
          \center{{\tiny ${0.000}$}}X
        \end{minipage}
        & \begin{minipage}{.12\linewidth}
          \includegraphics[width=\textwidth]{selem_results3/mnist_erosion_stick.png} \checkmark
          \vspace{-1cm}
          \center{{\tiny ${0.000}$}}
        \end{minipage}
        & \begin{minipage}{.12\linewidth}
          \includegraphics[width=\textwidth]{selem_results3/mnist_erosion_cross.png}
          \vspace{-1cm}
          \center{{\tiny ${0.000}$}}X
        \end{minipage}
        & \begin{minipage}{.12\linewidth}
          \includegraphics[width=\textwidth]{selem_results3/inverted_mnist_erosion_disk.png}X
          \vspace{-1cm}
          \center{{\tiny ${0.000}$}}
        \end{minipage}
        & \begin{minipage}{.12\linewidth}
          \includegraphics[width=\textwidth]{selem_results3/inverted_mnist_erosion_stick.png}O
          \vspace{-1cm}
          \center{{\tiny ${0.000}$}}
        \end{minipage}
        & \begin{minipage}{.12\linewidth}
          \includegraphics[width=\textwidth]{selem_results3/inverted_mnist_erosion_cross.png}X
          \vspace{-1cm}
          \center{{\tiny ${0.000}$}}
        \end{minipage}
        \\
        \hline
      \end{tabular}


==> results_table_opeclos.tex <==
     \begin{tabular}{ | c | c | c | c | c | c | c |}
        \hline
        Operation & Disk & Hstick & Vstick & Scross & Dcross & Square \\
        \hline
        Target
        & \begin{minipage}{.12\linewidth}
          \includegraphics[width=\textwidth]{selem_results/true_disk7.png}
        \end{minipage}
        & \begin{minipage}{.12\linewidth}
          \includegraphics[width=\textwidth]{selem_results/true_hstick7.png}
        \end{minipage}
        & \begin{minipage}{.12\linewidth}
          \includegraphics[width=\textwidth]{selem_results/true_vstick7.png}
  
        \end{minipage}
        & \begin{minipage}{.12\linewidth}
          \includegraphics[width=\textwidth]{selem_results/true_scross7.png}
        \end{minipage}
        & \begin{minipage}{.12\linewidth}
          \includegraphics[width=\textwidth]{selem_results/true_dcross7.png}
        \end{minipage}
        & \begin{minipage}{.12\linewidth}
          \includegraphics[width=\textwidth]{selem_results/true_square7.png}
        \end{minipage}
        \\        
        \hline
        Opening $\circ$
        & \begin{minipage}{.12\linewidth}
          \includegraphics[width=\textwidth]{selem_results/opening/opening_disk7_1.png} 
          \includegraphics[width=\textwidth]{selem_results/opening/opening_disk7_2.png}
          \vspace{-1cm}
          \center{{\tiny FAIRE}}
        \end{minipage}
        & \begin{minipage}{.12\linewidth}
          \includegraphics[width=\textwidth]{selem_results/opening/opening_hstick7_1.png}
          \includegraphics[width=\textwidth]{selem_results/opening/opening_hstick7_2.png}
          \vspace{-1cm}
          \center{{\tiny $1$}}
        \end{minipage}
        & \begin{minipage}{.12\linewidth}
          \includegraphics[width=\textwidth]{selem_results/opening/opening_vstick7_1.png}
          \includegraphics[width=\textwidth]{selem_results/opening/opening_vstick7_2.png}
          \vspace{-1cm}
          \center{{\tiny $1$}}
        \end{minipage}
        & \begin{minipage}{.12\linewidth}
          \includegraphics[width=\textwidth]{selem_results/opening/opening_scross7_1.png}
          \includegraphics[width=\textwidth]{selem_results/opening/opening_scross7_2.png}
          \vspace{-1cm}
          \center{{\tiny KO}}
        \end{minipage}
        & \begin{minipage}{.12\linewidth}
          \includegraphics[width=\textwidth]{selem_results/opening/opening_dcross7_1.png}
          \includegraphics[width=\textwidth]{selem_results/opening/opening_dcross7_2.png}
          \vspace{-1cm}
          \center{{\tiny $1$}}
        \end{minipage}
        & \begin{minipage}{.12\linewidth}
          \includegraphics[width=\textwidth]{selem_results/opening/opening_square7_1.png}
          \includegraphics[width=\textwidth]{selem_results/opening/opening_square7_2.png}
          \vspace{-1cm}
          \center{{\tiny $0.82$}}
        \end{minipage}
        \\
        \hline
        Closing $\bullet$
        & \begin{minipage}{.12\linewidth}
          \includegraphics[width=\textwidth]{selem_results/closing/closing_disk7_1.png}
          \includegraphics[width=\textwidth]{selem_results/closing/closing_disk7_2.png}
          \vspace{-1cm}
          \center{{\tiny $1$}}
        \end{minipage}
        & \begin{minipage}{.12\linewidth}
          \includegraphics[width=\textwidth]{selem_results/closing/closing_hstick7_1.png}
          \includegraphics[width=\textwidth]{selem_results/closing/closing_hstick7_2.png}
          \vspace{-1cm}
          \center{{\tiny $1$}}
        \end{minipage}
        & \begin{minipage}{.12\linewidth}
          \includegraphics[width=\textwidth]{selem_results/closing/closing_vstick7_1.png}
          \includegraphics[width=\textwidth]{selem_results/closing/closing_vstick7_2.png}
          \vspace{-1cm}
          \center{{\tiny $1$}}
        \end{minipage}
        & \begin{minipage}{.12\linewidth}
          \includegraphics[width=\textwidth]{selem_results/closing/closing_scross7_1.png}
          \includegraphics[width=\textwidth]{selem_results/closing/closing_scross7_2.png}
          \vspace{-1cm}
          \center{{\tiny $0.99$}}
        \end{minipage}
        & \begin{minipage}{.12\linewidth}
          \includegraphics[width=\textwidth]{selem_results/closing/closing_dcross7_1.png}
          \includegraphics[width=\textwidth]{selem_results/closing/closing_dcross7_2.png}
          \vspace{-1cm}
          \center{{\tiny $1$}}
        \end{minipage}
        & \begin{minipage}{.12\linewidth}
          \includegraphics[width=\textwidth]{selem_results/closing/closing_square7_1.png}
          \includegraphics[width=\textwidth]{selem_results/closing/closing_square7_2.png}
          \vspace{-1cm}
          \center{{\tiny $0.97$}}
        \end{minipage}
        \\
        \hline
      \end{tabular}


==> results_table_opeclos2.tex <==
     \begin{tabular}{ | c | c | c | c | c | c | c | c | c | c |}
        \hline
        Dataset & \multicolumn{3}{c|}{Diskorect}  & \multicolumn{3}{c|}{Mnist} & \multicolumn{3}{c|}{Inverted Mnist} \\
        \hline
        Operation & Disk & Hstick & Vstick & Scross & Dcross & Square & Scross & Dcross & Square \\
        \hline
        Target
        & \begin{minipage}{.12\linewidth}
          \includegraphics[width=\textwidth]{selem_results/true_disk7.png}
        \end{minipage}
        & \begin{minipage}{.12\linewidth}
          \includegraphics[width=\textwidth]{selem_results/true_hstick7.png}
        \end{minipage}
        & \begin{minipage}{.12\linewidth}
          \includegraphics[width=\textwidth]{selem_results/true_dcross7.png}
        \end{minipage}
        & \begin{minipage}{.12\linewidth}
          \includegraphics[width=\textwidth]{selem_results/true_disk7.png}
        \end{minipage}
        & \begin{minipage}{.12\linewidth}
          \includegraphics[width=\textwidth]{selem_results/true_hstick7.png}
        \end{minipage}
        & \begin{minipage}{.12\linewidth}
          \includegraphics[width=\textwidth]{selem_results/true_dcross7.png}
        \end{minipage}
        & \begin{minipage}{.12\linewidth}
          \includegraphics[width=\textwidth]{selem_results/true_disk7.png}
        \end{minipage}
        & \begin{minipage}{.12\linewidth}
          \includegraphics[width=\textwidth]{selem_results/true_hstick7.png}
        \end{minipage}
        & \begin{minipage}{.12\linewidth}
          \includegraphics[width=\textwidth]{selem_results/true_dcross7.png}
        \end{minipage}
        \\        
        \hline
        Opening $\circ$
        & \begin{minipage}{.12\linewidth}
          \includegraphics[width=\textwidth]{selem_results2/diskorect/opening/disk1.png} 
          \includegraphics[width=\textwidth]{selem_results2/diskorect/opening/disk2.png}
          \vspace{-1cm}
          \center{{\tiny $0.0001$}}
        \end{minipage}
        & \begin{minipage}{.12\linewidth}
          \includegraphics[width=\textwidth]{selem_results2/diskorect/opening/hstick1.png}
          \includegraphics[width=\textwidth]{selem_results2/diskorect/opening/hstick2.png}
          \vspace{-1cm}
          \center{{\tiny $0$}}
        \end{minipage}
        & \begin{minipage}{.12\linewidth}
          \includegraphics[width=\textwidth]{selem_results2/diskorect/opening/dcross1.png}
          \includegraphics[width=\textwidth]{selem_results2/diskorect/opening/dcross2.png}
          \vspace{-1cm}
          \center{{\tiny $0$}}
        \end{minipage}
        & \begin{minipage}{.12\linewidth}
          \includegraphics[width=\textwidth]{selem_results2/mnist/opening/disk1.png} 
          \includegraphics[width=\textwidth]{selem_results2/mnist/opening/disk2.png}
          \vspace{-1cm}
          \center{{\tiny $0.01$}}
        \end{minipage}
        & \begin{minipage}{.12\linewidth}
          \includegraphics[width=\textwidth]{selem_results2/mnist/opening/hstick1.png}
          \includegraphics[width=\textwidth]{selem_results2/mnist/opening/hstick2.png}
          \vspace{-1cm}
          \center{{\tiny $0$}}
        \end{minipage}
        & \begin{minipage}{.12\linewidth}
          \includegraphics[width=\textwidth]{selem_results2/mnist/opening/dcross1.png}
          \includegraphics[width=\textwidth]{selem_results2/mnist/opening/dcross2.png}
          \vspace{-1cm}
          \center{{\tiny $0.01$}}
        \end{minipage}
        & \begin{minipage}{.12\linewidth}
          \includegraphics[width=\textwidth]{selem_results2/inverted_mnist/opening/disk1.png} 
          \includegraphics[width=\textwidth]{selem_results2/inverted_mnist/opening/disk2.png}
          \vspace{-1cm}
          \center{{\tiny $0.01$}}
        \end{minipage}
        & \begin{minipage}{.12\linewidth}
          \includegraphics[width=\textwidth]{selem_results2/inverted_mnist/opening/hstick1.png}
          \includegraphics[width=\textwidth]{selem_results2/inverted_mnist/opening/hstick2.png}
          \vspace{-1cm}
          \center{{\tiny $0.001$}}
        \end{minipage}
        & \begin{minipage}{.12\linewidth}
          \includegraphics[width=\textwidth]{selem_results2/inverted_mnist/opening/dcross1.png}
          \includegraphics[width=\textwidth]{selem_results2/inverted_mnist/opening/dcross2.png}
          \vspace{-1cm}
          \center{{\tiny $0.01$}}
        \end{minipage}
        \\
        \hline
        Closing $\bullet$
        & \begin{minipage}{.12\linewidth}
          \includegraphics[width=\textwidth]{selem_results2/diskorect/closing/disk1.png}
          \includegraphics[width=\textwidth]{selem_results2/diskorect/closing/disk2.png}
          \vspace{-1cm}
          \center{{\tiny $0.03$}}
        \end{minipage}
        & \begin{minipage}{.12\linewidth}
          \includegraphics[width=\textwidth]{selem_results2/diskorect/closing/hstick1.png}
          \includegraphics[width=\textwidth]{selem_results2/diskorect/closing/hstick2.png}
          \vspace{-1cm}
          \center{{\tiny $0.01$}}
        \end{minipage}
        & \begin{minipage}{.12\linewidth}
          \includegraphics[width=\textwidth]{selem_results2/diskorect/closing/dcross1.png}
          \includegraphics[width=\textwidth]{selem_results2/diskorect/closing/dcross2.png}
          \vspace{-1cm}
          \center{{\tiny $0.02$}}
        \end{minipage}
        & \begin{minipage}{.12\linewidth}
          \includegraphics[width=\textwidth]{selem_results2/mnist/closing/disk1.png}
          \includegraphics[width=\textwidth]{selem_results2/mnist/closing/disk2.png}
          \vspace{-1cm}
          \center{{\tiny $0.01$}}
        \end{minipage}
        & \begin{minipage}{.12\linewidth}
          \includegraphics[width=\textwidth]{selem_results2/mnist/closing/hstick1.png}
          \includegraphics[width=\textwidth]{selem_results2/mnist/closing/hstick2.png}
          \vspace{-1cm}
          \center{{\tiny $0$}}
        \end{minipage}
        & \begin{minipage}{.12\linewidth}
          \includegraphics[width=\textwidth]{selem_results2/mnist/closing/dcross1.png}
          \includegraphics[width=\textwidth]{selem_results2/mnist/closing/dcross2.png}
          \vspace{-1cm}
          \center{{\tiny $0.01$}}
        \end{minipage}
        & \begin{minipage}{.12\linewidth}
          \includegraphics[width=\textwidth]{selem_results2/inverted_mnist/closing/disk1.png}
          \includegraphics[width=\textwidth]{selem_results2/inverted_mnist/closing/disk2.png}
          \vspace{-1cm}
          \center{{\tiny $0.01$}}
        \end{minipage}
        & \begin{minipage}{.12\linewidth}
          \includegraphics[width=\textwidth]{selem_results2/inverted_mnist/closing/hstick1.png}
          \includegraphics[width=\textwidth]{selem_results2/inverted_mnist/closing/hstick2.png}
          \vspace{-1cm}
          \center{{\tiny $0$}}
        \end{minipage}
        & \begin{minipage}{.12\linewidth}
          \includegraphics[width=\textwidth]{selem_results2/inverted_mnist/closing/dcross1.png}
          \includegraphics[width=\textwidth]{selem_results2/inverted_mnist/closing/dcross2.png}
          \vspace{-1cm}
          \center{{\tiny $0$}}
        \end{minipage}
        \\
        \hline
      \end{tabular}


==> results_table_opeclos4.tex <==
     \begin{tabular}{ | c | c | c | c | c | c | c | c | c | c |}
        \hline
        Dataset & \multicolumn{3}{c|}{Diskorect}  & \multicolumn{3}{c|}{MNIST} & \multicolumn{3}{c|}{Inverted MNIST} \\
        \hline
        Operation & Disk & Stick & Cross & Disk & Stick & Cross & Disk & Stick & Cross \\
        \hline
        Target
        & \begin{minipage}{.12\linewidth}
          \includegraphics[width=\textwidth]{selem_results/true_disk7.png}
        \end{minipage}
        & \begin{minipage}{.12\linewidth}
          \includegraphics[width=\textwidth]{selem_results/true_hstick7.png}
        \end{minipage}
        & \begin{minipage}{.12\linewidth}
          \includegraphics[width=\textwidth]{selem_results/true_dcross7.png}
        \end{minipage}
        & \begin{minipage}{.12\linewidth}
          \includegraphics[width=\textwidth]{selem_results/true_disk7.png}
        \end{minipage}
        & \begin{minipage}{.12\linewidth}
          \includegraphics[width=\textwidth]{selem_results/true_hstick7.png}
        \end{minipage}
        & \begin{minipage}{.12\linewidth}
          \includegraphics[width=\textwidth]{selem_results/true_dcross7.png}
        \end{minipage}
        & \begin{minipage}{.12\linewidth}
          \includegraphics[width=\textwidth]{selem_results/true_disk7.png}
        \end{minipage}
        & \begin{minipage}{.12\linewidth}
          \includegraphics[width=\textwidth]{selem_results/true_hstick7.png}
        \end{minipage}
        & \begin{minipage}{.12\linewidth}
          \includegraphics[width=\textwidth]{selem_results/true_dcross7.png}
        \end{minipage}
        \\        
        \hline
        Opening $\circ$
        & \begin{minipage}{.12\linewidth}
          \includegraphics[width=\textwidth]{selem_results3/diskorect_opening_disk1.png} 
          \includegraphics[width=\textwidth]{selem_results3/diskorect_opening_disk2.png}
          \vspace{-1cm}
          \center{{\tiny ${0.072}$}}
        \end{minipage}
        & \begin{minipage}{.12\linewidth}
          \includegraphics[width=\textwidth]{selem_results3/diskorect_opening_stick1.png}
          \includegraphics[width=\textwidth]{selem_results3/diskorect_opening_stick2.png}
          \vspace{-1cm}
          \center{{\tiny ${0.000}$}}
        \end{minipage}
        & \begin{minipage}{.12\linewidth}
          \includegraphics[width=\textwidth]{selem_results3/diskorect_opening_cross1.png}
          \includegraphics[width=\textwidth]{selem_results3/diskorect_opening_cross2.png}
          \vspace{-1cm}
          \center{{\tiny ${0.002}$}}
        \end{minipage}
        & \begin{minipage}{.12\linewidth}
          \includegraphics[width=\textwidth]{selem_results3/mnist_opening_disk1.png} 
          \includegraphics[width=\textwidth]{selem_results3/mnist_opening_disk2.png}
          \vspace{-1cm}
          \center{{\tiny ${0.008}$}}
        \end{minipage}
        & \begin{minipage}{.12\linewidth}
          \includegraphics[width=\textwidth]{selem_results3/mnist_opening_stick1.png}
          \includegraphics[width=\textwidth]{selem_results3/mnist_opening_stick2.png}
          \vspace{-1cm}
          \center{{\tiny ${0.000}$}}
        \end{minipage}
        & \begin{minipage}{.12\linewidth}
          \includegraphics[width=\textwidth]{selem_results3/mnist_opening_cross1.png}
          \includegraphics[width=\textwidth]{selem_results3/mnist_opening_cross2.png}
          \vspace{-1cm}
          \center{{\tiny ${0.001}$}}
        \end{minipage}
        & \begin{minipage}{.12\linewidth}
          \includegraphics[width=\textwidth]{selem_results3/inverted_mnist_opening_disk1.png} 
          \includegraphics[width=\textwidth]{selem_results3/inverted_mnist_opening_disk2.png}
          \vspace{-1cm}
          \center{{\tiny ${0.006}$}}
        \end{minipage}
        & \begin{minipage}{.12\linewidth}
          \includegraphics[width=\textwidth]{selem_results3/inverted_mnist_opening_stick1.png}
          \includegraphics[width=\textwidth]{selem_results3/inverted_mnist_opening_stick2.png}
          \vspace{-1cm}
          \center{{\tiny ${0.001}$}}
        \end{minipage}
        & \begin{minipage}{.12\linewidth}
          \includegraphics[width=\textwidth]{selem_results3/inverted_mnist_opening_cross1.png}
          \includegraphics[width=\textwidth]{selem_results3/inverted_mnist_opening_cross2.png}
          \vspace{-1cm}
          \center{{\tiny ${0.012}$}}
        \end{minipage}
        \\
        \hline
        Closing $\bullet$
        & \begin{minipage}{.12\linewidth}
          \includegraphics[width=\textwidth]{selem_results3/diskorect_closing_disk1.png}
          \includegraphics[width=\textwidth]{selem_results3/diskorect_closing_disk2.png}
          \vspace{-1cm}
          \center{{\tiny ${0.038}$}}
        \end{minipage}
        & \begin{minipage}{.12\linewidth}
          \includegraphics[width=\textwidth]{selem_results3/diskorect_closing_stick1.png}
          \includegraphics[width=\textwidth]{selem_results3/diskorect_closing_stick2.png}
          \vspace{-1cm}
          \center{{\tiny ${0.000}$}}
        \end{minipage}
        & \begin{minipage}{.12\linewidth}
          \includegraphics[width=\textwidth]{selem_results3/diskorect_closing_cross1.png}
          \includegraphics[width=\textwidth]{selem_results3/diskorect_closing_cross2.png}
          \vspace{-1cm}
          \center{{\tiny ${0.000}$}}
        \end{minipage}
        & \begin{minipage}{.12\linewidth}
          \includegraphics[width=\textwidth]{selem_results3/mnist_closing_disk1.png}
          \includegraphics[width=\textwidth]{selem_results3/mnist_closing_disk2.png}
          \vspace{-1cm}
          \center{{\tiny ${0.009}$}}
        \end{minipage}
        & \begin{minipage}{.12\linewidth}
          \includegraphics[width=\textwidth]{selem_results3/mnist_closing_stick1.png}
          \includegraphics[width=\textwidth]{selem_results3/mnist_closing_stick2.png}
          \vspace{-1cm}
          \center{{\tiny ${0.001}$}}
        \end{minipage}
        & \begin{minipage}{.12\linewidth}
          \includegraphics[width=\textwidth]{selem_results3/mnist_closing_cross1.png}
          \includegraphics[width=\textwidth]{selem_results3/mnist_closing_cross2.png}
          \vspace{-1cm}
          \center{{\tiny ${0.020}$}}
        \end{minipage}
        & \begin{minipage}{.12\linewidth}
          \includegraphics[width=\textwidth]{selem_results3/inverted_mnist_closing_disk1.png}
          \includegraphics[width=\textwidth]{selem_results3/inverted_mnist_closing_disk2.png}
          \vspace{-1cm}
          \center{{\tiny ${0.009}$}}
        \end{minipage}
        & \begin{minipage}{.12\linewidth}
          \includegraphics[width=\textwidth]{selem_results3/inverted_mnist_closing_stick1.png}
          \includegraphics[width=\textwidth]{selem_results3/inverted_mnist_closing_stick2.png}
          \vspace{-1cm}
          \center{{\tiny ${0.000}$}}
        \end{minipage}
        & \begin{minipage}{.12\linewidth}
          \includegraphics[width=\textwidth]{selem_results3/inverted_mnist_closing_cross1.png}
          \includegraphics[width=\textwidth]{selem_results3/inverted_mnist_closing_cross2.png}
          \vspace{-1cm}
          \center{{\tiny ${0.000}$}}
        \end{minipage}
        \\
        \hline
      \end{tabular}

==> structuring_elements.tex <==
     \begin{tabular}{ | c | c | c | c | c | c | c |}
        \hline
        Operation & Disk & Hstick & Vstick & Scross & Dcross & Square \\
        \hline
        Target
        & \begin{minipage}{.12\linewidth}
          \includegraphics[width=\textwidth]{selem_results/true_disk7.png}
        \end{minipage}
        & \begin{minipage}{.12\linewidth}
          \includegraphics[width=\textwidth]{selem_results/true_hstick7.png}
        \end{minipage}
        & \begin{minipage}{.12\linewidth}
          \includegraphics[width=\textwidth]{selem_results/true_vstick7.png}
  
        \end{minipage}
        & \begin{minipage}{.12\linewidth}
          \includegraphics[width=\textwidth]{selem_results/true_scross7.png}
        \end{minipage}
        & \begin{minipage}{.12\linewidth}
          \includegraphics[width=\textwidth]{selem_results/true_dcross7.png}
        \end{minipage}
        & \begin{minipage}{.12\linewidth}
          \includegraphics[width=\textwidth]{selem_results/true_square7.png}
        \end{minipage}
        \\
        \hline
      \end{tabular}


==> structuring_elements2.tex <==
     \begin{tabular}{ | c | c | c | c | c | c | c |}
        \hline
        % Dataset & \multicolumn{3}{c|}{Diskorect} & \multicolumn{3}{c|}{MNIST}
        Size & \multicolumn{3}{c|}{$7 \times 7$} & \multicolumn{3}{c|}{$5 \times 5$}\\
        \hline
        Operation & Disk & Stick & Cross & Disk & Stick & Cross \\
        \hline
        Target
        & \begin{minipage}{.12\linewidth}
          \includegraphics[width=\textwidth]{selem_results/true_disk7.png}
        \end{minipage}
        & \begin{minipage}{.12\linewidth}
          \includegraphics[width=\textwidth]{selem_results/true_hstick7.png}
        \end{minipage}
        & \begin{minipage}{.12\linewidth}
          \includegraphics[width=\textwidth]{selem_results/true_dcross7.png}
        \end{minipage}
        & \begin{minipage}{.12\linewidth}
          \includegraphics[width=\textwidth]{selem_results2/true_disk5.png}
        \end{minipage}
        & \begin{minipage}{.12\linewidth}
          \includegraphics[width=\textwidth]{selem_results2/true_hstick5.png}
        \end{minipage}
        & \begin{minipage}{.12\linewidth}
          \includegraphics[width=\textwidth]{selem_results2/true_dcross5.png}
        \end{minipage}
        \\
        \hline
      \end{tabular}

